Data-Driven Methods for Present and Future Pandemics: Monitoring, Modelling and Managing

This survey analyses the role of data-driven methodologies for pandemic modelling and control. We provide a roadmap from the access to epidemiological data sources to the control of epidemic phenomena. We review the available methodologies and discuss the challenges in the development of data-driven strategies to combat the spreading of infectious diseases. Our aim is to bring together several different disciplines required to provide a holistic approach to epidemic analysis, such as data science, epidemiology, and systems-and-control theory. A 3M-analysis is presented, whose three pillars are: Monitoring, Modelling and Managing. The focus is on the potential of data-driven schemes to address three different challenges raised by a pandemic: (i) monitoring the epidemic evolution and assessing the effectiveness of the adopted countermeasures; (ii) modelling and forecasting the spread of the epidemic; (iii) making timely decisions to manage, mitigate and suppress the contagion. For each step of this roadmap, we review consolidated theoretical approaches (including data-driven methodologies that have been shown to be successful in other contexts) and discuss their application to past or present epidemics, such as Covid-19, as well as their potential application to future epidemics.

==> Economics_and_Social_Modelling.tex <==

\section{Modelling economic and social impact }



\subsection{Economic Analysis}



Estimates and models produced at the time of the SARS outbreak suggested that it could have a catastrophic effect on the global economy. However, the scale of the SARS impact on affected economies was far smaller than contemporary media reports and model estimates \cite{Keogh-Brown2008}. More comprehensive macro-economic models providing better estimates of the relative cost and effect of a global, international responses to outbreaks is a open problem. This is specially the case for the COVID-19 outbreak. \cite{Baldwin2020Keeping}. 

In \cite{Johnson2020}, stock market volatility, newspaper-based economic uncertainty, and subjective uncertainty in business expectation surveys are used as indicators to document and quantify the enormous increase in economic uncertainty due to COVID-19 pandemic. The authors illustrate how these indicators could be used to assess  the macroeconomic impact of the COVID-19 using the model of disaster effects developed by Baker, Bloom and Terry (2020). 


% \begin{figure}[ht!]
%    \centering
%    \includegraphics[width=1.0\textwidth]{images/circular_flow_2.png}
%    \caption{Esta gráfica la podemos rehacer en Powerpoint o similar indicando dónde afecta el %Covid. Como en la siguiente que pongo aquí abajo.}
%    \label{fig:structure}
%\end{figure}
%\vspace{2mm}

%
%\begin{figure}[ht!]
%    \centering
%    \includegraphics[width=1.0\textwidth]{images/Circular_Flow_and_Covid19.JPG}
%    \caption{Algo así podríamos intentar. Otra opción es poner la gráfica 2 y enumerar en el %texto qué flujos se ven muy condicionados por el bichito \TEO{YA lo tengo, lo que se puede hacer %es hacer el dibujo de la gráfica anterior con las flechas con un color tanto más rojo, cuanto %más afectadas  estén con la pandemia } }
%    \label{fig:structure}
%\end{figure}
%\vspace{2mm}}


Modelos con gráficas: \cite{Baldwin2020Keeping}


\subsection{Some techniques for economic modelling}

\begin{itemize}
    \item Applications of catastrophe theory
\item Nonlinear dynamics of the response
\item Applications of dynamic systems
\item Modelling phase transitions
\item Models of self-organising criticality
\item Non-perturbative models of fat tails
\item Fractal models of crashes and contagion
\item Nonlinear spatial econometrics
\end{itemize}


Economic activity (growth, cycles)
Unemployment
Inequality
Public finances
High, middle and low income countries
The European integration process

